Analyzing Privacy Breaches in the Aircraft Communications Addressing and Reporting System (ACARS)

The manner in which Aircraft Communications, Addressing and Reporting System (ACARS) is being used has significantly changed over time. Whilst originally used by commercial airliners to track their flights and provide automated timekeeping on crew, today it serves as a multi-purpose air-ground data link for many aviation stakeholders including private jet owners, state actors and military. Since ACARS messages are still mostly sent in the clear over a wireless channel, any sensitive information sent with ACARS can potentially lead to a privacy breach for users. Naturally, different stakeholders consider different types of data sensitive. In this paper we propose a privacy framework matching aviation stakeholders to a range of sensitive information types and assess the impact for each. Based on more than one million ACARS messages, collected over several months, we then demonstrate that current ACARS usage systematically breaches privacy for all stakeholder groups. We further support our findings with a number of cases of significant privacy issues for each group and analyze the impact of such leaks. While it is well-known that ACARS messages are susceptible to eavesdropping attacks, this work is the first to quantify the extent and impact of privacy leakage in the real world for the relevant aviation stakeholders.

==> README <==
                 The dgruyter package:                 
preparing books and journals for Walter de Gruyter GmbH


File:       README
Author:     le-tex publishing services


DESCRIPTION
===========

The dgruyter package assists in preparing manuscripts for de Gruyter
with {\LaTeX}. It provides some special commands for journal papers
as well as for books and generates the required appearance.
Together with corresponding font packages it allows to produce the 
final layout of De Gruyter books and journal articles.

Copyright:  (C) 2015, 2016 Walter de Gruyter GmbH


FILES IN DISTRIBUTION
=====================

   BASE DISTRIBUTION:

      README                  This file.
      dgruyter.ins            Package installation file.
      dgruyter.dtx            Package source file.
      dg-degruyter.eps/.pdf   Logo files.
      dg-mouton.eps/.pdf      Logo files.
      dg-saur.eps/.pdf        Logo files.
      DG_attention.eps/.pdf   Vignette files.
      DG_exercise.eps/.pdf    Vignette files.
      DG_information.eps/.pdf Vignette files.
      DG_notice.eps/.pdf      Vignette files.
      DG_question.eps/.pdf    Vignette files.
      book.tex                Template file for a book.
      article.tex             Template file for a journal article.

   DOCUMENTATIONs:

      dgruyter.pdf            User manual for dgruyter package. 
                              It is produced as described below.

      dgruyter-faqs.pdf      Frequently asked questions to dgruyter.sty


BASIC INSTALLATION
====================

   To get the package style file 'dgruyter.sty' and the
   index style files 'dgruyter.ist' and 'dgruyter.xdy' execute:
     latex dgruyter.ins

   The minimum requirement to use the package is to have
     dgruyter.sty and dgruyter.ist/dgruyter.xdy
     (as well as the logo and vignette files)
     in a directory where TeX can find it.

   To get the documentation 'dgruyter.pdf' execute:
     pdflatex dgruyter.dtx (at least twice)


==> paper (copy)/README <==
                 The dgruyter package:                 
preparing books and journals for Walter de Gruyter GmbH


File:       README
Author:     le-tex publishing services


DESCRIPTION
===========

The dgruyter package assists in preparing manuscripts for de Gruyter
with {\LaTeX}. It provides some special commands for journal papers
as well as for books and generates the required appearance.
Together with corresponding font packages it allows to produce the 
final layout of De Gruyter books and journal articles.

Copyright:  (C) 2015, 2016 Walter de Gruyter GmbH


FILES IN DISTRIBUTION
=====================

   BASE DISTRIBUTION:

      README                  This file.
      dgruyter.ins            Package installation file.
      dgruyter.dtx            Package source file.
      dg-degruyter.eps/.pdf   Logo files.
      dg-mouton.eps/.pdf      Logo files.
      dg-saur.eps/.pdf        Logo files.
      DG_attention.eps/.pdf   Vignette files.
      DG_exercise.eps/.pdf    Vignette files.
      DG_information.eps/.pdf Vignette files.
      DG_notice.eps/.pdf      Vignette files.
      DG_question.eps/.pdf    Vignette files.
      book.tex                Template file for a book.
      article.tex             Template file for a journal article.

   DOCUMENTATIONs:

      dgruyter.pdf            User manual for dgruyter package. 
                              It is produced as described below.

      dgruyter-faqs.pdf      Frequently asked questions to dgruyter.sty


BASIC INSTALLATION
====================

   To get the package style file 'dgruyter.sty' and the
   index style files 'dgruyter.ist' and 'dgruyter.xdy' execute:
     latex dgruyter.ins

   The minimum requirement to use the package is to have
     dgruyter.sty and dgruyter.ist/dgruyter.xdy
     (as well as the logo and vignette files)
     in a directory where TeX can find it.

   To get the documentation 'dgruyter.pdf' execute:
     pdflatex dgruyter.dtx (at least twice)

